Multifidelity Covariance Estimation via Regression on the Manifold of Symmetric Positive Definite Matrices

We introduce a multifidelity estimator of covariance matrices formulated as the solution to a regression problem on the manifold of symmetric positive definite matrices. The estimator is positive definite by construction, and the Mahalanobis distance minimized to obtain it possesses properties enabling practical computation. We show that our manifold regression multifidelity (MRMF) covariance estimator is a maximum likelihood estimator under a certain error model on manifold tangent space. More broadly, we show that our Riemannian regression framework encompasses existing multifidelity covariance estimators constructed from control variates. We demonstrate via numerical examples that the MRMF estimator can provide significant decreases, up to one order of magnitude, in squared estimation error relative to both single-fidelity and other multifidelity covariance estimators. Furthermore, preservation of positive definiteness ensures that our estimator is compatible with downstream tasks, such as data assimilation and metric learning, in which this property is essential.

==> figures/sqg_metricLearning/sqg_classA_final.tex <==
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  \let\gplgaddtomacro\g@addto@macro
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3739,4051){\makebox(0,0)[r]{\strut{}observation points}}%
      \csname LTb\endcsname%
      \put(1757,667){\makebox(0,0){\strut{}$-3$}}%
      \put(2264,667){\makebox(0,0){\strut{}$-2$}}%
      \put(2772,667){\makebox(0,0){\strut{}$-1$}}%
      \put(3279,667){\makebox(0,0){\strut{}$0$}}%
      \put(3786,667){\makebox(0,0){\strut{}$1$}}%
      \put(4294,667){\makebox(0,0){\strut{}$2$}}%
      \put(4801,667){\makebox(0,0){\strut{}$3$}}%
      \put(1446,1138){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(1446,1645){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(1446,2153){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(1446,2660){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1446,3167){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1446,3675){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(1446,4182){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(5448,1066){\makebox(0,0)[l]{\strut{}$-1$}}%
      \put(5448,1597){\makebox(0,0)[l]{\strut{}$-0.8$}}%
      \put(5448,2128){\makebox(0,0)[l]{\strut{}$-0.6$}}%
      \put(5448,2659){\makebox(0,0)[l]{\strut{}$-0.4$}}%
      \put(5448,3191){\makebox(0,0)[l]{\strut{}$-0.2$}}%
      \put(5448,3722){\makebox(0,0)[l]{\strut{}$0$}}%
      \put(5448,4254){\makebox(0,0)[l]{\strut{}$0.2$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{sqg_classA_final}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/sqg_metricLearning/sqg_classA_init.tex <==
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  \let\gplgaddtomacro\g@addto@macro
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1757,667){\makebox(0,0){\strut{}$-3$}}%
      \put(2264,667){\makebox(0,0){\strut{}$-2$}}%
      \put(2772,667){\makebox(0,0){\strut{}$-1$}}%
      \put(3279,667){\makebox(0,0){\strut{}$0$}}%
      \put(3786,667){\makebox(0,0){\strut{}$1$}}%
      \put(4294,667){\makebox(0,0){\strut{}$2$}}%
      \put(4801,667){\makebox(0,0){\strut{}$3$}}%
      \put(1446,1138){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(1446,1645){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(1446,2153){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(1446,2660){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1446,3167){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1446,3675){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(1446,4182){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(5448,1066){\makebox(0,0)[l]{\strut{}$-1$}}%
      \put(5448,1384){\makebox(0,0)[l]{\strut{}$-0.9$}}%
      \put(5448,1703){\makebox(0,0)[l]{\strut{}$-0.8$}}%
      \put(5448,2022){\makebox(0,0)[l]{\strut{}$-0.7$}}%
      \put(5448,2341){\makebox(0,0)[l]{\strut{}$-0.6$}}%
      \put(5448,2659){\makebox(0,0)[l]{\strut{}$-0.5$}}%
      \put(5448,2978){\makebox(0,0)[l]{\strut{}$-0.4$}}%
      \put(5448,3297){\makebox(0,0)[l]{\strut{}$-0.3$}}%
      \put(5448,3616){\makebox(0,0)[l]{\strut{}$-0.2$}}%
      \put(5448,3935){\makebox(0,0)[l]{\strut{}$-0.1$}}%
      \put(5448,4254){\makebox(0,0)[l]{\strut{}$0$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{sqg_classA_init}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/sqg_metricLearning/sqg_classB_final.tex <==
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  \let\gplgaddtomacro\g@addto@macro
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3739,4051){\makebox(0,0)[r]{\strut{}observation points}}%
      \csname LTb\endcsname%
      \put(1757,667){\makebox(0,0){\strut{}$-3$}}%
      \put(2264,667){\makebox(0,0){\strut{}$-2$}}%
      \put(2772,667){\makebox(0,0){\strut{}$-1$}}%
      \put(3279,667){\makebox(0,0){\strut{}$0$}}%
      \put(3786,667){\makebox(0,0){\strut{}$1$}}%
      \put(4294,667){\makebox(0,0){\strut{}$2$}}%
      \put(4801,667){\makebox(0,0){\strut{}$3$}}%
      \put(1446,1138){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(1446,1645){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(1446,2153){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(1446,2660){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1446,3167){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1446,3675){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(1446,4182){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(5448,1066){\makebox(0,0)[l]{\strut{}$-1.2$}}%
      \put(5448,1597){\makebox(0,0)[l]{\strut{}$-1$}}%
      \put(5448,2128){\makebox(0,0)[l]{\strut{}$-0.8$}}%
      \put(5448,2659){\makebox(0,0)[l]{\strut{}$-0.6$}}%
      \put(5448,3191){\makebox(0,0)[l]{\strut{}$-0.4$}}%
      \put(5448,3722){\makebox(0,0)[l]{\strut{}$-0.2$}}%
      \put(5448,4253){\makebox(0,0)[l]{\strut{}$0$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{sqg_classB_final}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/sqg_metricLearning/sqg_classB_init.tex <==
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  \let\gplgaddtomacro\g@addto@macro
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1757,667){\makebox(0,0){\strut{}$-3$}}%
      \put(2264,667){\makebox(0,0){\strut{}$-2$}}%
      \put(2772,667){\makebox(0,0){\strut{}$-1$}}%
      \put(3279,667){\makebox(0,0){\strut{}$0$}}%
      \put(3786,667){\makebox(0,0){\strut{}$1$}}%
      \put(4294,667){\makebox(0,0){\strut{}$2$}}%
      \put(4801,667){\makebox(0,0){\strut{}$3$}}%
      \put(1446,1138){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(1446,1645){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(1446,2153){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(1446,2660){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1446,3167){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1446,3675){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(1446,4182){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(5448,1066){\makebox(0,0)[l]{\strut{}$-1$}}%
      \put(5448,1384){\makebox(0,0)[l]{\strut{}$-0.9$}}%
      \put(5448,1703){\makebox(0,0)[l]{\strut{}$-0.8$}}%
      \put(5448,2022){\makebox(0,0)[l]{\strut{}$-0.7$}}%
      \put(5448,2341){\makebox(0,0)[l]{\strut{}$-0.6$}}%
      \put(5448,2659){\makebox(0,0)[l]{\strut{}$-0.5$}}%
      \put(5448,2978){\makebox(0,0)[l]{\strut{}$-0.4$}}%
      \put(5448,3297){\makebox(0,0)[l]{\strut{}$-0.3$}}%
      \put(5448,3616){\makebox(0,0)[l]{\strut{}$-0.2$}}%
      \put(5448,3935){\makebox(0,0)[l]{\strut{}$-0.1$}}%
      \put(5448,4254){\makebox(0,0)[l]{\strut{}$0$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={360.00bp},height={252.00bp}]{sqg_classB_init}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> xx.tex <==



==> yy.tex <==


